Non-forking and preservation of NIP and dp-rank

We investigate the question of whether the restriction of a NIP type $p\in S(B)$ which does not fork over $A\subseteq B$ to $A$ is also NIP, and the analogous question for dp-rank. We show that if $B$ contains a Morley sequence $I$ generated by $p$ over $A$, then $p\restriction AI$ is NIP and similarly preserves the dp-rank. This yields positive answers for generically stable NIP types and the analogous case of stable types. With similar techniques we also provide a new more direct proof for the latter. Moreover, we introduce a general construction of "trees whose open cones are models of some theory" and in particular an inp-minimal theory DTR of dense trees with random graphs on open cones, which exemplifies a negative answer to the question.

==> Final32Type.tex <==
% !TEX root = FinalPreservationNiP.tex

%NOTAS!!!!!!!!!!!!!!!!!!!!!!!!!!!!____________________________________________________


%¿Se puede mejorar la escritura en general?!!!!!!!!!!!!!!!
%Está bien 
%
%------------------------------------------------------------------------------------- 
 
\begin{comment}
\subsection{The type}
\label{sec:32}
We set notation for the next two sections. Let $M\models DTR$ be a model with $\mathfrak{C}$ the monster, and $B$ a branch of $M$ (a maximal chain), consider the partial type $\rho(x)=\Set{x>b}{b\in B}$. 

\begin{prop}\label{prop:rho determines a complete type} $\rho$ determines a unique complete type $q(x)$ over $M$.\end{prop}
\begin{proof} For every $m \in M \setminus{B}$, there is some $b \in B$ such that $b \not < m$, and it follows that $\rho\vdash x \wedge m = b \wedge m$. This implies that $\rho$ already determines a complete type over $M$ in the language of trees $\{\leq, \wedge\}$. 

Next we determine all formulas of the form $\chi = R(t_0(x,m), t_1(x,m), t_2(x,m))$ where $m$ is a tuple from $M$. By the previous paragraph, for any term $t(x,m)$, $\rho \vdash t(x,m) = x$ or $\rho \vdash t(x,m) = m_t$ where $m_t$ is an element from $M$. If $t_0 = x$, then $\rho \models \neg \chi$ (because it cannot be that $t_0 \wedge t_1 = x < t_0,t_1$). If all terms are already in $M$ there is nothing to do, so by symmetry (\textit{i.e.} (R2)), the only remaining case is when $t_0 = m_0$, $t_1 = x$ are from $M$ and $t_2 = m_2$ where $\rho \vdash x \wedge m_2 = m_0 \mathop{\&} m_0 < x, m_2$ and in particular $m_0 \in B$ and $m_2 \notin B$. Let $b \in B$ be such that $b \not < m_2$. Then by (R3), as $\rho \vdash m_0<b = b \wedge x$, it follows that $\rho \vdash \chi \leftrightarrow R(m_0,b,m_2)$. \end{proof}

\begin{prop} \label{prop:q has IP} $q(x)\in S(M)$ has IP. \end{prop} 
    \begin{proof} Let $d\models q$ and $(b_i)_{i<\omega}$ a sequence of realizations of $q$ such that $b_i\wedge b_j=d$ for all $i\neq j$. By (RGC) (see Lemma \ref{lem:rgc holds}), for every $s\subseteq\omega$ we have that $\Gamma_s(x)=\Set{x \wedge b_i = d \mathop{\&} R(d,x,b_i)^{(i\in s)}}{i<\omega}$ is consistent. Of course, any realization of $\Gamma_s$ also realizes $\rho$ and hence $q$ (by Proposition \ref{prop:rho determines a complete type}). Together, we have that 
    for every such $s \subseteq \omega$, $q(x) \cup \Set{R(x \wedge b_i,x,b_i)^{(i\in s)}}{i<\omega}$ is consistent, meaning that $q$ has IP. 
\end{proof}
    
    %: Given $R(x\wedge b_1,x,b_n)\dots, R(x\wedge b_n,x,b_n),\lnot R(x\wedge b_{n+1},x,b_{n+1}),\dots, \lnot R(x\wedge b_{n+m},x,b_{n+m})$ by the property $(RGC)$ of the theory DTR we can find an element $a$ in a new open cone of center $d$ satisfying $\models\mathop{\&}_{i=1}^n R(d,a,b_i)$ and $\models\mathop{\&}_{i=n+1}^{n+m}\lnot R(d,a,b_i)$. This implies $d=a\wedge b_i$ for $i=1,\dots,n+m$. Hence $\models\mathop{\&}_{i=1}^n R(a\wedge b_i,a,b_i)$ and $\models\mathop{\&}_{i=n+1}^{n+m}\lnot R(a\wedge b_i,a,b_i)$ as we want. Therefore we have IP.\end{proof}


Let $c\models q$ in $\mathfrak{C}$ and $\pi(x)=q(x)\cup\{x<c\}$. 

\begin{prop} $\pi(x)$ does not fork over $M$ and moreover it is finitely satisfiable in $M$ (in fact in $B$).\end{prop}

\begin{proof} This follows from Proposition \ref{prop:rho determines a complete type}, as $\pi(x)$ is equivalent to $\rho(x)\cup \{x<c\}$. \end{proof}

%Clearly the set determines all formulas in $\{\leq, \wedge\}$. 

%For those of kind $R(t_1(x,\bar{m}), t_2(x,\bar{m}), t_3(x,\bar{m}))$: First note that if $a\models\Set{x>b}{b\in B}$, then $a\wedge m=m$ for every $m\in B$. And if $m\in M\smallsetminus B$, then $a\wedge m=m'$ for $m'\in B$ such that $m\wedge m'=m'$. Hence, the terms $x\wedge m$ are equivalent to $m'$. Moreover note that if $\models R(a,m_1,m_2)$, then $a<m_1, m_2$ and this is a contradiction, since for every point $m\in M$, $a>m$ or $a$ and $m$ are incomparable. Hence it only remains to check whether the formulas $R(m_1,x,m_2)$ are determined. We only need the following information: for each $b\in B$ a subset $\mathcal{A}_b$ of the set of open cones of center $b$, meaning that $\Set{x>b'}{b'\in B}\vdash R(b,x,m)$ for every $m$ in each open cone in $\mathcal{A}_b$ and $\Set{x>b'}{b'\in B}\vdash\lnot R(b,x,m)$ otherwise. But $\models R(b,a,m)$ is equivalent to $\models R(b,b',m)$ for every $b'\in B$ such that $b'>b$, because $a, b'$ are in the same open cone of center $b$. Thus it is determined by $M$.\end{proof}





\begin{prop} \label{pro:pi is NIP} $\pi(x)$ is NIP.\end{prop}
\begin{proof} Towards a contradiction, suppose we have an $Mc$-indiscernible sequence $I = (b_i)_{i<\omega}$, a formula $\varphi(x,y)$ and $a\models\pi(x)$ such that $\models\varphi(a,b_i)^{(\,i\,\mbox{even})}$. In particular, $\varphi$ has IP. By quantifier elimination, we may assume that $\varphi$ is quantifier free. As NIP-formulas are closed under Boolean combinations by \textit{e.g.} \cite[Lemma 2.9]{Sim}, and as DT is NIP (Fact \ref{fac:dt}) and is the reduct of DTR to the tree language (Remark \ref{rem:DTR = DT + RGC}), we may assume that $\varphi(x,y)=R(t_0(x,y),t_1(x,y),t_2(x,y))$, for some terms $t_0,t_1,t_2$.

    Let $J = (c_i)_{i<\omega}$ with $c_i = (b_{2i}b_{2i+1})$. By Ramsey and compactness, there is an $Mca$-indiscernible sequence $J' = (c_i)_{i<\omega_1}$ such that $EM(J'/Mca) \subseteq EM(J/Mca)$. Note that we still have $\models\varphi(a,b'_i)^{(\,i\,\mbox{even})}$ where $c'_i = (b'_{2i}b'_{2i+1})$ and that $I'=(b'_i)_{i<{\omega_1}}$ is $Mc$-indiscernible. As DT is NIP, there is a final segment of $I'$ which is $Mca$-indiscernible in the language of trees (see Remark \ref{rem:alternation}). Replacing $I$ with an infinite subsequence of that final segment, we may assume that $I$ is $Mac$-indiscernible in the language of trees. 

    Since $\models R\left(t_0(a,b_i),t_1(a,b_i),t_2(a,b_i)\right)^{(\,i\,\mbox{even})}$, we know that $t_0(a, b_i) = t_1(a,b_i) \wedge t_2(a,b_i) < t_1(a,b_i), t_2(a,b_i)$ for $i$ even, and by indiscernibility in the tree language, this is always true. 

    If $x$ does not appear in any of $t_0,t_1,t_2$, there is nothing to do. If $x$ does not appear in both $t_1,t_2$, then as $t_0(a, b_i) = t_1(a,b_i) \wedge t_2(a,b_i)$, we can replace $t_0$ by $t_1 \wedge t_2$ and we can reduce to the previous case. Assume without loss of generality that $x$ appears in $t_1$ (otherwise use symmetry). Note that in general, if $x$ appears in a term $t(x,b)$, then $t(a,b) \leq a$, so we necessarily get that $t_1(a,b_i)\leq a <c$ for all $i<\omega$.  On the other hand, it cannot be that $x$ appears in both $t_1,t_2$, since then $t_1(a,b_i),t_2(a,b_i)$ are comparable, contradicting the previous paragraph. So $x$ does not appear in $t_2$. It follows that $t_0(a,b_i) = t_1(a,b_i) \wedge t_2(b_i) = c \wedge t_2(b_i)$.
    %(by induction on $t$)
    
    
Finally, by (R3), it follows that $R\left(t_0(a,b_i),t_1(a,b_i),t_2(a,b_i)\right) \leftrightarrow R\left(c \wedge t_2(b_i),c,t_2(b_i)\right)$, and as $(b_i)_{i<\omega}$ is $c$-indiscernible, $\varphi(a,b_i)$ has a constant truth value, contradiction. \end{proof}

    
    

    
    
    %We may assume $\varphi(x,y)=R\left(t_1(x,y),t_2(x,y),t_3(x,y)\right)$, where $t_l(x,y)$ are terms of the language. Indeed, since DTR has QE any formula $\varphi(x,y)$ is a finite boolean combination of atomic formulas $\psi_{i,j}(x,y)$, and by the pigeonhole principle if $\varphi(x,y)$ has infinite alternation so does some $\psi_{i,j}(x,y)$. Moreover as we know that the theory DT is NIP (Fact \ref{fac:dt}), these are the unique kind of atomic formulas that remain to check.
 
  
 %We may assume \quad $(*)$\, $t_1(a, b_i)< t_2(a,b_i), t_3(a,b_i)$ for all $i<\omega$:
 
 %Since $\models R\left(t_1(a,b_i),t_2(a,b_i),t_3(a,b_i)\right)^{(\,i\,\mbox{even})}$, by the axioms of $DTR_R$ we know that $t_1(a, b_i)< t_2(a,b_i), t_3(a,b_i)$ for $i$ even. Now, since $\alpha(x,y):=\left(t_1(x,y)<t_2(x,y)\right)\land\left(t_1(x,y)<t_3(x,y)\right)$ is NIP it can only have a finite number of alternations and since $\models\alpha(a,b_i)$ for $i$ even we have $\models\alpha(a,b_i)$ eventually.
 

 %Moreover we may assume\quad $(**)$\, $t_1(a,b_i)=t_2(a,b_i)\wedge t_3(a,b_i)$ for all $i<\omega$.
 
 %This is because we have $t_1(a, b_i)\leq t_2(a,b_i)\wedge t_3(a,b_i)$ and if $t_1(a, b_i)< t_2(a,b_i)\wedge t_3(a,b_i)$ then $\models\lnot R\left(t_1(a,b_i),t_2(a,b_i),t_3(a,b_i)\right)$, but since $R$ holds for the even indices and the formula $\alpha(x,y):=\left(t_1(x,y)=\left(t_2(x,y)\wedge t_3(x,y)\,\right)\,\right)$ is NIP, we have $\models\alpha(a,b_i)$ eventually.
 
   
 %Note that $x$ must occur in some of the terms $t_l(x,y)$, $l=2,3$. Otherwise $t_l(x,y)=t_l(y)$ for $l=2, 3$ and then $t_1(a,b_i)=t_2(b_i)\wedge t_3(b_i)$ depends only on $b_i$, \textit{i.e.} $t_1(a,b_i)=t_1(b_i)$. Thus we have $\models R\left(t_1(b_i),t_2(b_i),t_3(b_i)\right)^{(\,i\,\mbox{even})}$ which is a contradiction with the fact of $(b_i)_{i<\omega}$ indiscernible. Since the terms are finitely many meet operation symbols $t_l(a,b_i)\leq a$ for some $l=2,3$, in particular $t_1(a,b_i)< a <c$ for all $i<\omega$.
 

 %If $x$ occurs in both $t_2(x,y), t_3(x,y)$, then $t_1(a,b_i)<t_2(a,b_i), t_3(a,b_i)\leq a$ for every $i<\omega$. So for each $i$ it can be that they are all distinct or $t_2(a,b_i)=t_3(a,b_i)$. In any case we get a contradiction with $(**)$. Therefore $x$ does not occur in some term. Since $R(u,v,w)$ is symmetric in $v,w$ we may assume that $t_3(x,y)=t_3(y)$.
 

 %Now $x$ must occur in $t_2(x,y)$, hence $t_2(a,b_i)\leq a<c$. Since the formula $\alpha(x,y):=t_2(x,y)<t_3(y)$ is NIP we may assume: either $t_2(a,b_i)<t_3(b_i)$ for all $i<\omega$ \,or $t_2(a,b_i)>t_3(b_i)$ for all $i<\omega$ \, or $t_2(a,b_i),\, t_3(b_i)$ incomparable for all $i<\omega$. In the first two cases we get a contradiction, since $t_1(a, b_i)< t_2(a,b_i), t_3(b_i)$ by $(*)$ and on the other hand $t_1(a,b_i)$ equals to some of $t_2(a,b_i), t_3(b_i)$ by $(**)$. In the last one $t_1(a,b_i)=t_2(a,b_i)\wedge t_3(b_i)=c\wedge t_3(b_i)$ and also $c\wedge t_2(a,b_i)=t_2(a,b_i)>t_1(a,b_i)$. Therefore we have $\models R\left(t_1(a,b_i),t_2(a,b_i),t_3(a,b_i)\right)$ if and only if $\models R\left(t_3(b_i)\wedge c, c, t_3(b_i)\right)$  which is a contradiction since $(b_i)_{i<\omega}$ is $Mc$-indiscernible. \end{proof} 
 

\begin{cor} The answer to Question \ref{question} is negative. \end{cor}

\begin{rk} Note that the question was phrased for complete types, but by taking a non-forking or even a coheir extension we can find such a type. 
    
Also, note that as we cannot hope that our counterexample is definable over a model by Corollary \ref{cor:positive2}; the next best thing is a coheir, which is what we have. \end{rk}

% Therefore we can extend $\pi$ to a global coheir $\mathfrak{p}$, thus an $M$-invariant type (whose restriction is $q(x)$). As we are going to see, $\pi$ is NIP and so is $\mathfrak{p}$. Hence this example is not only an answer for the general question about forking, but in particular for invariant types. Recall that the subclass of definable global types is a positive example (Corollary \ref{cor:positive2}), but we are showing a coheir in DTR which is a negative one.

\end{comment}
